PromptGate Client Adaptive Vision Language Gating for Open Set Federated Active Learning

Deploying medical AI across resource-constrained institutions demands data-efficient learning pipelines that respect patient privacy. Federated Learning (FL) enables collaborative medical AI without centralising data, yet real-world clinical pools are inherently open-set, containing out-of-distribution (OOD) noise such as imaging artifacts and wrong modalities. Standard Active Learning (AL) query strategies mistake this noise for informative samples, wasting scarce annotation budgets. We propose PromptGate, a dynamic VLM-gated framework for Open-Set Federated AL that purifies unlabeled pools before querying. PromptGate introduces a federated Class-Specific Context Optimization: lightweight, learnable prompt vectors that adapt a frozen BiomedCLIP backbone to local clinical domains and aggregate globally via FedAvg -- without sharing patient data. As new annotations arrive, prompts progressively sharpen the ID/OOD boundary, turning the VLM into a dynamic gatekeeper that is strategy-agnostic: a plug-and-play pre-selection module enhancing any downstream AL strategy. Experiments on distributed dermatology and breast imaging benchmarks show that while static VLM prompting degrades to 50% ID purity, PromptGate maintains $>$95% purity with 98% OOD recall.

==> sections_arxiv/annexes.tex <==
\section*{Annexes}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/fedisic_farood/Legend_AL_Methods.png} \\
    % %\vspace{0.2cm}
    \includegraphics[width=0.32\textwidth]{figures/fedisic_farood/shaded/BMA_AL_Baseline.png}
    \includegraphics[width=0.32\textwidth]{figures/fedisic_farood/shaded/QR_AL_Baseline.png}
    \includegraphics[width=0.32\textwidth]{figures/fedisic_farood/shaded/AQR_AL_Baseline.png} \\
    % %\vspace{0.4cm}
    \includegraphics[width=0.32\textwidth]{figures/fedisic_farood/shaded/BMA_AL_CSC_G8-L8_Mixed.png}
    \includegraphics[width=0.32\textwidth]{figures/fedisic_farood/shaded/QR_AL_CSC_G8-L8_Mixed.png}
    \includegraphics[width=0.32\textwidth]{figures/fedisic_farood/shaded/AQR_AL_CSC_G8-L8_Mixed.png}
    \caption{Comparison of AL methods on FedISIC FarOOD 50\% under the VLM-Static baseline (top row) versus our proposed CSC G8-L8 Mixed variant (bottom row).}
    \label{fig:farood_al_comparison}
\end{figure*}



% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/fedembed/Legend_VLM_Variants.png} \\
%     %\vspace{0.2cm}
%     % Use \hfill to evenly space the three images and prevent line wrapping
%     \includegraphics[width=0.32\textwidth]{figures/fedembed/noshading/BMA_VLM_Variants.png}\hfill
%     \includegraphics[width=0.32\textwidth]{figures/fedembed/noshading/QR_VLM_Variants.png}\hfill
%     \includegraphics[width=0.32\textwidth]{figures/fedembed/noshading/AQR_VLM_Variants.png}
%     \caption{Average BMA over labeled data, QP, and AQR across all AL methods for different VLM filter variants on FedEMBED.}
%     \label{fig:fedembed_vlm_variants}
% \end{figure*}

\begin{figure*}[t!]
   \centering
   \includegraphics[width=0.9\textwidth]{figures/fedisic_farood/Legend_AL_Methods.png} \\
    %\vspace{0.2cm}
    \includegraphics[width=0.32\textwidth]{figures/fedembed_noshading/BMA_AL_Baseline.png}\hfill
    \includegraphics[width=0.32\textwidth]{figures/fedembed_noshading/QR_AL_Baseline.png}\hfill
    \includegraphics[width=0.32\textwidth]{figures/fedembed_noshading/AQR_AL_Baseline.png} \\
    %\vspace{0.4cm}
    \includegraphics[width=0.32\textwidth]{figures/fedembed_noshading/BMA_AL_CSC_G8-L8_Mixed.png}\hfill
    \includegraphics[width=0.32\textwidth]{figures/fedembed_noshading/QR_AL_CSC_G8-L8_Mixed.png}\hfill
    \includegraphics[width=0.32\textwidth]{figures/fedembed/AQR_AL_CSC_G8-L8_Mixed.png}\hfill
    \caption{Comparison of AL methods on FedEMBED under the VLM-Static baseline (top row) versus our proposed CSC G8-L8 Mixed variant (bottom row). Average BMA over AL Round, QP, and QP are shown.}
   \label{fig:fedembed_al_comparison}
\end{figure*}



\begin{table}[h]
\centering
\caption{VLM Test Set Performance on FedISIC for the Random acquisition strategy at AL Round 15. We display the per-client and overall performance metrics comparing the Global, Local, and Mixed CSC variants against the non-adapted Static model.}
\label{tab:fedisic_test_vlm_performance}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{clccccc}
\toprule
\textbf{VLM Variant} & \textbf{Metric (\%)} & \textbf{Client 0} & \textbf{Client 1} & \textbf{Client 2} & \textbf{Client 3} & \textbf{Overall} \\
\midrule
\multirow{4}{*}{\textbf{Global}}
 % & ID Purity & \textbf{99.7} & 100.0 & \textbf{99.9} & 99.9 & \textbf{99.8} \\
 & ID BMA      & 33.9 & 62.9 & \textbf{44.9} & 36.7 & 41.8 \\
 & Accuracy & \textbf{99.6} & 99.6 & \textbf{99.7} & \textbf{99.9} & \textbf{99.6} \\
 & OOD Recall  & 97.9 & 99.7 & \textbf{99.3} & 99.1 & 98.5 \\
\midrule
\multirow{4}{*}{\textbf{Local}}
 % & ID Purity   & \textbf{99.8} & \textbf{100.0} & \textbf{99.9} & \textbf{99.9} & \textbf{99.8} \\
 & ID BMA      & 32.5 & 55.4 & 44.7 & \textbf{38.9} & 40.1 \\
 & Accuracy & \textbf{99.6} & 99.4 & \textbf{99.7} & 99.8 & \textbf{99.6} \\
 & OOD Recall  & \textbf{98.3} & \textbf{100.0} & 99.0 & \textbf{99.1} & \textbf{98.8} \\
\midrule
\multirow{4}{*}{\textbf{Mixed}}
 % & ID Purity   & 99.7 & \textbf{100.0} & \textbf{99.9} & 99.6 & 99.7 \\
 & ID BMA      & \textbf{35.7} & \textbf{64.4} & 43.2 & 35.3 & \textbf{42.0} \\
 & Accuracy & 99.5 & 99.6 & \textbf{99.7} & 99.7 & \textbf{99.6} \\
 & OOD Recall  & 97.6 & 99.7 & \textbf{99.3} & 97.6 & 98.2 \\
\midrule
\multirow{4}{*}{\textbf{Baseline}}
 % & ID Purity   & 86.9 & 88.0 & 86.9 & 86.0 & 87.0 \\
 & ID BMA      & 30.6 & 27.6 & 31.2 & 26.6 & 27.5 \\
 & Accuracy & 83.2 & 87.9 & 85.8 & 82.4 & 84.4 \\
 & OOD Recall  & 0.6 & 0.9 & 0.0 & 0.0 & 0.5 \\
\bottomrule
\end{tabular}
}\end{table}

Table~\ref{tab:fedisic_test_vlm_performance} shows that learnable variants provide massive absolute gains over the \emph{Baseline}. \emph{Mixed} improves ID Purity by 12.7\%, Binary Accuracy by 15.2\%, and ID BMA by 14.5\% absolute. While the \emph{Baseline} fails to filter artifacts (0.5\% OOD Recall), all learnable versions reach $>98$\% recall—a 97.7\% absolute jump. Among variants, \emph{Local} is most robust in filtering (+0.6\% OOD Recall over \emph{Mixed}), yet \emph{Mixed} delivers the best task performance, outperforming \emph{Local} by 1.9\% and \emph{Global} by 0.2\% in BMA. Finally, while the Task Model maintains a higher overall BMA (66.3\%), the adapted VLM serves as its essential open-set gatekeeper, recovering a 14\% relative performance drop caused by artifact leakage in the baseline.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/fedisic_farood/vlm_test/Legend_VLM_Variants.png} \\
    %\vspace{0.2cm}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client0_id_balanced_acc.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client1_id_balanced_acc.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client2_id_balanced_acc.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client3_id_balanced_acc.png} \\
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client0_ood_accuracy.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client1_ood_accuracy.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client2_ood_accuracy.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client3_ood_accuracy.png} \\
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client0_ood_recall_ood.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client1_ood_recall_ood.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client2_ood_recall_ood.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test/Client3_ood_recall_ood.png}
    \caption{Per-client VLM test set performance (ID BMA, Accuracy, and OOD Recall) across AL rounds for different VLM filter variants on FedISIC. Rows represent metrics (ID BMA, Accuracy, OOD Recall) and columns represent Clients 0 to 3.}
    \label{fig:fedisic_vlm_test_per_client}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/fedisic_farood/vlm_test/Legend_VLM_Variants.png} \\
    %\vspace{0.2cm}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client0_id_balanced_acc.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client0_id_balanced_acc.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client2_id_balanced_acc.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client3_id_balanced_acc.png} \\
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client0_ood_accuracy.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client1_ood_accuracy.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client2_ood_accuracy.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client3_ood_accuracy.png} \\
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client0_ood_recall_ood.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client1_ood_recall_ood.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client2_ood_recall_ood.png}
    \includegraphics[width=0.24\textwidth]{figures/fedisic_farood/vlm_test_with_baseline/Client3_ood_recall_ood.png}
    \caption{Per-client VLM test set performance (ID BMA, Accuracy, and OOD Recall) across AL rounds for different VLM filter variants on FedISIC, compared against the Static model (Baseline). Rows represent metrics (ID BMA, Accuracy, OOD Recall) and columns represent Clients 0 to 3.}
    \label{fig:fedisic_vlm_test_per_client}
\end{figure*}


